Transparent Object Tracking with Enhanced Fusion Module

Accurate tracking of transparent objects, such as glasses, plays a critical role in many robotic tasks such as robot-assisted living. Due to the adaptive and often reflective texture of such objects, traditional tracking algorithms that rely on general-purpose learned features suffer from reduced performance. Recent research has proposed to instill transparency awareness into existing general object trackers by fusing purpose-built features. However, with the existing fusion techniques, the addition of new features causes a change in the latent space making it impossible to incorporate transparency awareness on trackers with fixed latent spaces. For example, many of the current days transformer-based trackers are fully pre-trained and are sensitive to any latent space perturbations. In this paper, we present a new feature fusion technique that integrates transparency information into a fixed feature space, enabling its use in a broader range of trackers. Our proposed fusion module, composed of a transformer encoder and an MLP module, leverages key query-based transformations to embed the transparency information into the tracking pipeline. We also present a new two-step training strategy for our fusion module to effectively merge transparency features. We propose a new tracker architecture that uses our fusion techniques to achieve superior results for transparent object tracking. Our proposed method achieves competitive results with state-of-the-art trackers on TOTB, which is the largest transparent object tracking benchmark recently released. Our results and the implementation of code will be made publicly available at https://github.com/kalyan0510/TOTEM.

==> figures/attb_neg.tex <==
\begin{figure}[t!]
        \centering
        \begin{subfigure}{0.45\textwidth}
            \centering
            \includegraphics[width=\linewidth]{src/attb_oov1.eps}
            \caption[Out of View]%
            {{\small Out of View}}    
            % \label{fig:mean and std of net14}
            \label{fig:sotacmpsuc}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.45\textwidth}  
            \centering 
            \includegraphics[width=\linewidth]{src/attb_foc1.eps}
            \caption[Full Occlusion]%
            {{\small Full Occlusion}}    
            % \label{fig:mean and std of net24}
            \label{fig:sotacmpnpe}
        \end{subfigure}
        \caption[  Analysis over tracking challenges: Out of View, and Full Occlusion  ]
        {\small Tracking performance of different tracking algorithms over the attributes on which adding transparency features have negative impact in terms of success metric. (Legend shows values in rate unit)
        } 
        \label{fig:attbneg}
    \end{figure}

==> tables/attb_anlz.tex <==
\begin{table*}[!t]
\centering

% % \makebox[\textwidth][c]{
%     \begin{tabular}{lcccccc}
% \toprule
% %       &       & \multicolumn{3}{c}{CCSHR\_11} & \multicolumn{3}{c}{CCSHR\_12} \\
% % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%           &  IV  &  POC & DEF  &  MB  &  ROT &  BC  \\ \midrule
% TOTEM (diff. w/ TOMP)     & \textbf{82.2} (7.1↑) & \textbf{71.4} (4.3↑) & \textbf{79.2} (13↑) & \textbf{69.5} (4↑) & \textbf{73.8} (3.5↑) & \textbf{69.4} (1.3↑) \\
% TOMP      & 75.1 & 67.1 & 66.2 & 65.5 & 70.3 & 68.1 \\ 
% TOMP-finetuned & 77.8 & 69.1 & 71.6 & 67.8 & 71.8 & 67.6\\ \hdashline
% TransATOM & 66.9 & 58.0 & 64.0 & 52.5 & 60.0 & 59.6 \\
% ATOM      & 62.6 & 55.6 & 58.6 & 50.0 & 55.3 & 58.1 \\
% \bottomrule
% \end{tabular}%
% % }

% % \makebox[\textwidth][c]{
%     \begin{tabular}{lcccccc}
% %       &       & \multicolumn{3}{c}{CCSHR\_11} & \multicolumn{3}{c}{CCSHR\_12} \\
% % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% &  SV  &  FOC &  FM  &  OV  &  LR  & ARC \\ \midrule
% TOTEM (diff. w/ TOMP)  & \textbf{74.5} (6.2↑) & 41.1 (5.3↓)& \textbf{68.1} (8.2↑) & 60.9 2(.5↓) & \textbf{74.0} (10.9↑) & \textbf{73.5} (6.4↑) \\
% TOMP   & 68.3 & \textbf{46.4} & 59.9 & \textbf{61.4} & 63.1 & 67.1 \\ 
% TOMP-finetuned & 70.1 & 41.1 & 63.8 & 59.9 & 64.3 & 68.5\\  \hdashline
% TransATOM & 59.6 & 27.6 & 50.0 & 36.5 & 58.3 & 58.4\\
% ATOM & 53.8 & 31.6 & 45.4 & 40.0 & 58.7 & 50.9\\
% \bottomrule
% \end{tabular}%
% \end{table}
% % }





\makebox[\textwidth][c]{
    \begin{tabular}{lccccccccccccc}
\toprule
%       &       & \multicolumn{3}{c}{CCSHR\_11} & \multicolumn{3}{c}{CCSHR\_12} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}
          & All  &  IV  &  POC & DEF  &  MB  &  ROT &  BC  &  SV  &  FOC &  FM  &  OV  &  LR  & ARC \\ \midrule
TOMP      & 70.0 & 75.1 & 67.1 & 66.2 & 65.5 & 70.3 & 68.1 & 68.3 & \textbf{46.4} & 59.9 & \textbf{61.4} & 63.1 & 67.1\\
TransATOM & 62.2 & 66.9 & 58.0 & 64.0 & 52.5 & 60.0 & 59.6 & 59.6 & 27.6 & 50.0 & 36.5 & 58.3 & 58.4\\
ATOM      & 58.6 & 62.6 & 55.6 & 58.6 & 50.0 & 55.3 & 58.1 & 53.8 & 31.6 & 45.4 & 40.0 & 58.7 & 50.9\\
TOTEM(Ours)     & \textbf{75.6} & \textbf{82.2} & \textbf{71.4} & \textbf{79.2} & \textbf{69.5} & \textbf{73.8} & \textbf{69.4} & \textbf{74.5} & 41.1 & \textbf{68.1} & 60.9 & \textbf{74.0} & \textbf{73.5}\\
\bottomrule
\end{tabular}%
}

\caption{Per attribute analysis on TOTB Test split. Value in each cell corresponds to success AUC metric (in \%) corresponding to the tracker and attribute. TOTEM scores the best against all the tracking challenges except \textit{Full-Occlusion} and \textit{Out-of-View}}

\label{table:perattbanlzXXX}%
\end{table*}%


==> tables/baseline_ablate.tex <==
\begin{table}[!t]
\centering
% \makebox[\textwidth][c]{
    \begin{tabular}{lccc}
\toprule
Baseline Trackers                                & SUC   &  PE  & NPE \\ \midrule
                                % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}

TOMP                          & 70.0      & 72.2          & 80.7 \\ 
ATOM                          & 58.6      & 59.0          & 68.4 \\ 
DiMP                          & 56.5      & 54.5          & 62.7 \\ \midrule
TransATOM                     & 61.4 & 61.7 & 71.4 \\

\bottomrule
\end{tabular}%
% }
\caption{Analysis of different backbones for tracking performance
on TOTB using SUC score. These results are extracted from the work of their respective authors (except for TOMP which we tested on TOTB split)}

\label{table:ablatebaselineXXX}%
\end{table}%


==> tables/fusion_ablate.tex <==
\begin{table}[!t]
\centering
\makebox[\linewidth][c]{
    \begin{tabular}{lccc}
\toprule
Fusion approaches                               & SUC   &  PE  & NPE \\ \midrule
                                % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}

TOTEM-MLPHead    & 66.3      & 67.8 & 77.4 \\
TOTEM-Emb   & 69.7      &  \textbf{73.1}             & 81.4\\
TOTEM-FFNFuse             & 67.7      &  69.3                 & 79.4\\
TOTEM                      & \textbf{70.2}      &  72.9                 & \textbf{82.4}\\
\bottomrule
\end{tabular}%
}
\caption{Analysis of fusion module on tracking performance. }

\label{table:ablatefusionmoduleXXX}%
\end{table}%


==> tables/onetwo.tex <==
\begin{table*}
  \mbox{}\hfill
  \begin{minipage}[t]{.65\linewidth}
  \setlength\tabcolsep{2pt}
    \centering{\small
    \begin{tabular}{lccccccccccccc}
            \toprule
                      & All  &  IV  &  POC & DEF  &  MB  &  ROT &  BC  &  SV  &  FOC &  FM  &  OV  &  LR  & ARC \\ \midrule
            TOMP      & 70.0 & 75.1 & 67.1 & 66.2 & 65.5 & 70.3 & 68.1 & 68.3 & \textbf{46.4} & 59.9 & \textbf{61.4} & 63.1 & 67.1\\
            TransATOM & 62.2 & 66.9 & 58.0 & 64.0 & 52.5 & 60.0 & 59.6 & 59.6 & 27.6 & 50.0 & 36.5 & 58.3 & 58.4\\
            ATOM      & 58.6 & 62.6 & 55.6 & 58.6 & 50.0 & 55.3 & 58.1 & 53.8 & 31.6 & 45.4 & 40.0 & 58.7 & 50.9\\
            TOTEM(Ours)     & \textbf{75.6} & \textbf{82.2} & \textbf{71.4} & \textbf{79.2} & \textbf{69.5} & \textbf{73.8} & \textbf{69.4} & \textbf{74.5} & 41.1 & \textbf{68.1} & 60.9 & \textbf{74.0} & \textbf{73.5}\\
            \bottomrule
        \end{tabular}}

        \caption{\small Per attribute analysis on TOTB Test split. Value in each cell corresponds to success AUC metric (in \%) corresponding to the tracker and attribute. TOTEM scores the best against all the tracking challenges except \textit{Full-Occlusion} and \textit{Out-of-View}}
        \label{table:onetwo/attb}
  \end{minipage}\hfill
  \begin{minipage}[t]{.25\linewidth}
    \centering
      \setlength\tabcolsep{2pt}

    \begin{tabular}{lccc}
            \toprule
            Baseline Trackers                                & SUC   &  PE  & NPE \\ \midrule
                                            % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}
            
            TOMP                          & \textbf{70.0}      & \textbf{72.2}          & \textbf{80.7} \\ 
            ATOM                          & 58.6      & 59.0          & 68.4 \\ 
            DiMP                          & 56.5      & 54.5          & 62.7 \\ \midrule
            TransATOM                     & 61.4 & 61.7 & 71.4 \\
            
            \bottomrule
            \end{tabular}

            \caption{\small Analysis of different backbones for tracking performance on TOTB using SUC score.}
        \label{table:onetwo/baseline}
            
  \end{minipage}\hfill
  \mbox{}
  \label{table:onetwo}
\end{table*}

==> tables/train_ablate.tex <==
\begin{table}[!t]
\centering
% \makebox[\textwidth][c]{
    \begin{tabular}{lccc}
\toprule
Training methods                                & SUC   &  PE  & NPE \\ \midrule
                                % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}

Two step train                          & 71.3      & 74.7          & 83.0 \\ 
One step train                          & 70.2      & 72.9          & 82.4 \\ \midrule
Two step + Model Pred. fine-tune             & 75.6      & 81.4          & 87.8 \\

\bottomrule
\end{tabular}%
% }
\caption{Analysis of training approach on tracking performance. }
\label{table:ablatetwosteptrainXXX}%
\end{table}%


==> tables/trans_ablate.tex <==
\begin{table}[!t]
\centering
% \makebox[\textwidth][c]{
    \begin{tabular}{lccc}
\toprule
                                & SUC   &  PE  & NPE \\ \midrule
                                % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}

TOTEM-TE                           & 70.4      & 72.9          & 81.3 \\
TOTEM-T                               & 70.3      & 72.7          & 81.8\\
TOTEM             & \textbf{75.6}      & \textbf{81.4}          & \textbf{87.8}\\


\bottomrule
\end{tabular}%
% }
\caption{Analysis of transparency features on tracking performance. }


%\minipage

\label{table:ablatetransfeatXXX}%
\end{table}%


==> tables/twoandthree.tex <==
\begin{table*}
  \begin{minipage}[t]{.25\linewidth}
  \setlength\tabcolsep{3pt}
    \centering{
    %%
        \begin{tabular}{lccc}
            \toprule
                                            & SUC   &  PE  & NPE \\ \midrule
                                            % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}
            
            TOTEM-TE                           & 70.4      & 72.9          & 81.3 \\
            TOTEM-T                               & 70.3      & 72.7          & 81.8\\
            TOTEM             & \textbf{75.6}      & \textbf{81.4}          & \textbf{87.8}\\
            
            
            \bottomrule
            \end{tabular}%
    }

    \caption{\small Analysis of transparency features on tracking performance. }
    \label{table:ablatetransfeat}%
  \end{minipage}\hfill
  \begin{minipage}[t]{.3\linewidth}
  \setlength\tabcolsep{2pt}
    \centering
    %%    
    \begin{tabular}{lccc}
    \toprule
    Fusion approaches                               & SUC   &  PE  & NPE \\ \midrule
                                    % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}
    TOTEM-MLPHead    & 66.3      & 67.8 & 77.4 \\
    TOTEM-\(e_\mathrm{query}\)   & 69.7      &  \textbf{73.1}             & 81.4\\
    TOTEM-FFNFuse             & 67.7      &  69.3                 & 79.4\\
    TOTEM                      & \textbf{70.2}      &  72.9                 & \textbf{82.4}\\
    \bottomrule
    \end{tabular}%

    \caption{\small Analysis of fusion module on tracking performance. }
    \label{table:ablatefusionmodule}%
  \end{minipage}\hfill
  \begin{minipage}[t]{.4\linewidth}
  \setlength\tabcolsep{2pt}

    \centering
    %%
        \begin{tabular}{lccc}
        \toprule
        Training methods                                & SUC   &  PE  & NPE \\ \midrule
                                        % & \multicolumn{3}{c}{AUC} \\  \cmidrule{2-4}
        One step train                          & 70.2      & 72.9          & 82.4 \\
        Two step train                          & 71.3      & 74.7          & 83.0 \\  \midrule
        Two step train + end-to-end fine-tune             & \textbf{75.6}      & \textbf{81.4}          & \textbf{87.8} \\
        
        \bottomrule
        \end{tabular}

    \caption{\small Analysis of training approach on tracking performance. }
    \label{table:ablatetwosteptrain}%
  \end{minipage}
\end{table*}

